Imaging current flow and injection in scalable graphene devices through NV-magnetometry

The global electronic properties of solid-state devices are strongly affected by the microscopic spatial paths of charge carriers. Visualising these paths in novel devices produced by scalable processes would provide a quality assessment method that can propel the device performance metrics towards commercial use. Here, we use high-resolution nitrogen-vacancy (NV) magnetometry to visualise the charge flow in gold-contacted, single-layer graphene devices produced by scalable methods. Modulating the majority carrier type via field effect reveals a strong asymmetry between the spatial current distributions in the electron and hole regimes that we attribute to an inhomogeneous microscopic potential landscape, inaccessible to conventional measurement techniques. In addition, we observe large, unexpected, differences in charge flow through nominally identical gold-graphene contacts. Moreover, we find that the current transfer into the graphene occurs several microns before the metal contact edge. Our findings establish high-resolution NV-magnetometry as a key tool for characterizing scalable 2D material based devices, uncovering quality deficits of the material, substrate, and electrical contacts that are invisible to conventional methods.

==> clippings.tex <==
intoduction bulletpoints:

\begin{itemize}
    \item 2D-material(particularly graphene) electronics and their importance for the future semicon and other industries \cite{IRDS2022,lemme2014two, liu2021promises, fiori2014electronics, zeng2021electronics, lemme20222d, du2014rm}
    \item challenges associated with developing 2DM electronics in particular with respect to graphene - with particular emphasis on contact resistance being poorly understood and measured. various methods suggested to reduce contact resistance \cite{lee2008contact,min2014improvement, xia2011origins, nagashio2010contact, nagashio2009metal}
    \item Our non-invasive, in-situ way of measuring current density on graphene
    \item We measure on different contact geometry of graphene providing information about current injection, homogeneity of contacts etc..
\end{itemize}



Figures \ref{fig:channel2}(a)-(b) also show the absence of current in the top and bottom corners of the gold contacts near the channel. This suggests that the current is injected in the graphene before the contact edge; this is in contrast with the current crowding mechanism \cmt{cite current crowding}.


\cmt{
what are the conclusions?/ things to add/extra thoughts:
\begin{itemize}
    \item is the transfer length dependent on the contact resistance? I mean also when there is only one contact? we could make a reference to horizontal line plots that show less currents where there are defects?
    \item can we say anything about edge injection vs basal plane injection? 
    \begin{itemize}
        \item if there would predominantly be edge injection, would we see more current in the gold near the edges of the graphene at the contacts? (would the current queue to reach the edge?)
        \item In the finger prong, we do not see that the transfer length equals the entire length of the graphene contact. Could this be a result of edge injection? (bias currents are the same)
        \item Defect in the contact = more edge = lower RC? (finger prongs)
        \item  this line was in the old text: \textit{The current also preferentially flows via the graphene edges indicating edge injection of charge carriers to be the main mechanism rather than basal plane injection.}, how do we draw this conclusions?
        \item what to do with the following sentence (part of the old text): \textit{Increasing the contact edge length has been shown to reduce the contact resistance of metal-graphene interface\cite{smith2013reducing, passi2019ultralow, min2014improvement, choi2022recent}.}
    \end{itemize}
    \item descriptions of the saw tooth feels a bit weak at the moment, what more can be extracted? (yes one can have expected more current in the gold than in the graphene, but something else?)
    \item what makes one contact more resistive than another? any ideas? (the top finger has more dark spots/less uniformity)
\end{itemize}
}
